Exploring Modality Guidance to Enhance VFM-based Feature Fusion for UDA in 3D Semantic Segmentation

Vision Foundation Models (VFMs) have become a de facto choice for many downstream vision tasks, like image classification, image segmentation, and object localization. However, they can also provide significant utility for downstream 3D tasks that can leverage the cross-modal information (e.g., from paired image data). In our work, we further explore the utility of VFMs for adapting from a labeled source to unlabeled target data for the task of LiDAR-based 3D semantic segmentation. Our method consumes paired 2D-3D (image and point cloud) data and relies on the robust (cross-domain) features from a VFM to train a 3D backbone on a mix of labeled source and unlabeled target data. At the heart of our method lies a fusion network that is guided by both the image and point cloud streams, with their relative contributions adjusted based on the target domain. We extensively compare our proposed methodology with different state-of-the-art methods in several settings and achieve strong performance gains. For example, achieving an average improvement of 6.5 mIoU (over all tasks), when compared with the previous state-of-the-art.

==> fig_tex/aggregate_performance_supplementory.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{img/aggregate_performance.png}
    \caption{Comparison to an alternative prediction aggregation for the final prediction. 
      We compare the softmax average of our VFM classifier and the fusion main classifier when added to the 3D prediction.}
    \label{fig:aggregate_performance}
\end{figure}

==> fig_tex/compare_model_performance_supplementory.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{img/vfm_comparison.png}
    \caption{Comparison of current SOTA VFMs on USA $\to$ Sing. and VK $\to$ SK. 
             We report the mIoU \% for our main heads including the VFM head utilized for the fusion regularization.}
    \label{fig:vfm_comparison_supplementory}
\end{figure}

==> tables/classes_supplementory.tex <==
\begin{table*}[t!]
\centering
\begin{tabular}{c|c}
\toprule
\textbf{Task}                 &  \textbf{Merged Classes}                           \\ \midrule
nuScenes derivations                  & Vehicle, Drivable Surface, Sidewalk, Terrain, Manmade, Vegetation    \\     

A2D2 $\to$ SK          & Car, Truck, Bike, Person, Road, Parking, Sidewalk, Building, Nature, Other-Objects                      \\ 
VK $\to$ SK    & Car, Truck, Road, Vegetation/Terrain, Building, Object                                                   \\ 
\bottomrule

\end{tabular}
\caption{List of classes for each task (excluding ignore and unlabeled classes). Both \emph{Day $\to$ Night} and \emph{USA $\to$ Singapore} use the same class mapping. }
\label{tab:merged_classes_tasks}
\end{table*}

==> tables/compare_to_xmuda_supplementory.tex <==
\begin{table}[t!]
\footnotesize
  \centering
\begin{tabular}{l|c|c|c}
\toprule
    2D3D  & USA $\to$ Sing. & Day $\to$ Night &  A2D2 $\to$ SK \\ 
     \midrule \midrule%\cline{2-5} 

xMUDA \cite{jaritz2022cross}  & 69.2 & 67.4 &  44.0 \\
xMUDA-Fuse \cite{jaritz2022cross}  &  69.3 & -  & 42.6  \\
xMUDA-VFM & 63.2 & 69.1  & 53.7  \\
xMUDA-VFM-F. & 73.4 & 64.1   & 61.4 \\
\midrule
Ours   & 74.6 & 70.3 &  63.1 \\ 
\bottomrule
\bottomrule
\end{tabular}
\caption{Extended comparison of xMUDA and xMUDA-Fuse variants with and without VFM backbone. For xMUDA-VFM and xMUDA-VFM-Fuse the trainable 2D backbone is replaced with a frozen VFM. For xMUDA-VFM the cross modal predictive alignment is applied on the 2D main head.  }

\label{tab:xmuda_supplementory_comparison}
\end{table}

==> tables/head_comparison_supplementory.tex <==
\begin{table*}
\centering
\small
{\begin{tabular}{l|cc|cc|cc|cc}
\toprule 
        & \multicolumn{2}{c}{USA $\to$ Singapore}
        & \multicolumn{2}{c}{Day $\to$ Night} 
        & \multicolumn{2}{c}{VK $\to$ SK} 
        & \multicolumn{2}{c}{A2D2 $\to$ SK}  \\ 
Method & VFM3D & 2D3D & VFM3D & 2D3D  & VFM3D & 2D3D & VFM3D & 2D3D   \\  \midrule \midrule%\cline{2-5} 
ours & 73.3 & 75.4 & 65.8 & 70.3 & 69.2& 70.7 & 61.3 & 63.1 \\
\end{tabular}}
\caption{Comparison of our heads} 
\label{tab:head_comparision}
\end{table*}

==> tables/source_ablation_supplementory.tex <==
\begin{table}
%\small
  \centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|ccc}
\toprule
   \multirow{2}{*}{Method}  & \multicolumn{3}{c}{VK $\to$ SK}\\ 
 &  2D & 3D & 2D3D  \\  \midrule\midrule%\cline{2-5} 
Source \cite{jaritz2022cross} & 26.8 & 42.0 & 42.2 \\
Source w\textbackslash o MG &  64.0 &  32.5 &  59.4\\
Source + MG &  64.9 &  29.0 &  59.9 \\ 
\midrule
Ours & 70.1 & 64.5 & 70.7\\ 

\bottomrule
\bottomrule
\end{tabular}%}
\caption{Source comparison. The regularizing effect of the modality guidance (MG) is setting in full when the target data is applied. }
\label{tab:source_comparision}
\end{table}

==> tables/tasks_splits_supplementroy_2.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l|c|ccc}
\toprule
\multirow{2}{*}{Task} & \multicolumn{1}{c}{Source} & \multicolumn{3}{c}{Target} \\
& Train & Train & Val & Test \\
\midrule
\midrule
USA $\to$ Sing. & 15,695 & 9,665 & 2,770 & 2,929 \\
Day $\to$ Night & 24,745 & 2,779 & 606 & 602 \\
VK $\to$ SK & 2,126 & 18,029 & 1,101 & 4,071 \\
A2D2 $\to$ SK & 27,695 & 18,029 & 1,101 & 4,071 \\
\bottomrule
\bottomrule
\end{tabular}
\caption{ Number of images per dataset split per task. }
\label{tab:dataset_task_splits}
\end{table}

